Data Enrichment Opportunities for Distribution Grid Cable Networks using Variational Autoencoders

Electricity distribution cable networks suffer from incomplete and unbalanced data, hindering the effectiveness of machine learning models for predictive maintenance and reliability evaluation. Features such as the installation date of the cables are frequently missing. To address data scarcity, this study investigates the application of Variational Autoencoders (VAEs) for data enrichment, synthetic data generation, imbalanced data handling, and outlier detection. Based on a proof-of-concept case study for Denmark, targeting the imputation of missing age information in cable network asset registers, the analysis underlines the potential of generative models to support data-driven maintenance. However, the study also highlights several areas for improvement, including enhanced feature importance analysis, incorporating network characteristics and external features, and handling biases in missing data. Future initiatives should expand the application of VAEs by incorporating semi-supervised learning, advanced sampling techniques, and additional distribution grid elements, including low-voltage networks, into the analysis.

==> sections/99_workflow.tex <==


\section{Opportunities for Data Enrichment with VAEs}
%%CHatGPT
This section introduces the structured algorithms and techniques forming the data enrichment workflow, with a focus on applicability beyond the current work. The methodology comprises two steps: the first involves conventional data preprocessing, encompassing strategies like data appending, feature engineering, outlier detection, and missing value removal; the second step addresses data scarcity, class imbalance, and missing value imputation through a deep generative model based on VAEs. While tailored to the specific problem, this approach's universal mathematical framework and architectural structure enhance its adaptability across diverse scenarios with minimal modifications.

The initial phase involves a comprehensive examination of well-established data preprocessing techniques in the context of ML algorithms, known for improving training stability, robustness, and model performance, followed by the introduction of methods potentially valuable to DSOs for data preparation. The techniques used in this work can be listed as missing value and outlier removal, external data appending, feature selection and feature generation. While some of these are self-explanatory, the rest will be elaborated on later in the sections using the dataset of interest in this work.

%%ChatGPT
While the first stage of the preprocessing pipeline suits many datasets for ML model training, additional requirements are necessary in some cases. The focus is on exploring VAEs, where a foundation is laid by understanding deep generative models (DGMs) and model-based approaches. These concepts combine to define VAEs' unique properties, which will be further explained to demonstrate their effectiveness in addressing common data challenges and contributing as a tool for managing real-world ML issues.

%%ChatGPT
Deep Generative Models (DGMs) are neural networks with hidden layers trained to mimic complex probability distributions, aiming to capture elusive distributions from limited samples. Effectively trained DGMs can estimate sample likelihood and generate resembling samples, serving as a solution for data augmentation. Unlike traditional methods like SMOTE, DGMs accurately represent the true data distribution and have proven valuable in enhancing models, particularly for smaller subgroups. Additionally, DGMs address missing value imputation by learning underlying data distribution and generating plausible data points based on feature correlations.


==> sections/results.tex <==


% \section{Results and Discussion}



% \subsection{Results: title might be removed later}

% % \textcolor{red}{Describe the general capability of the VAE to reproduce distributions in line with the input data. Insert images of age training data distribution and real distribution. Show values for metrices. }
% % Text here 
% % Figure XX exemplary visualises the cumulative distribution functions of the continuous features: Age, humidity (past1h), and temperature (past1h). This  VAE is able to adjust correctly the statistical distribution when sampling new synthetic observations.



% \textcolor{red}{Describe the general capabilities if the CVAE to reproduce target feature distributions. Show how the feature distributions are different from each other. Show values for metrics. }
%  Figures XX, XX, and XX show the results of the CVAEs distribution per component type. 
% \textcolor{red}{
% Provide reconstruction error for different features and missing values --> Show that the reconstruction works of individual values works. That similar values lead to similar reconstructions. Alternatively train a classification model on }
% Text here 

% \subsection{Amputation of Missing Age information}
% \textcolor{red}{Apply the process of missing values imputation on "faked" missing entries. Impute values in the training data and show that the generall process works}
% One possibility to evaluate the usability of the CVAE to impute missing values in the dataset is given by amputation. For this, a random mask is defined for a feature where missing values are to be expected. 
% This enables the comparison of estimated and real values after imputation. One highly important but frequently missing feature is the age of the cable during failure. Therefore it has been selected to test the CVAE imputation capability. In order to benchmark the results of the CVAE-based imputation, the same amputation task has been fulfilled with another State of Art Imputation Algorithm, MissForest. 

% \textcolor{red}{Consider the integration of other imputation algorithms such as the KNN Imputer}

% As seen in Figure X and X lack both MVI methods 
% are capable of identifying the two peaks in cable ages during failure. However, both lack the capability of imputing cable failures over 60 years. Thus, they systematically underestimate the cable age and failures of older cables. In particular, for the MissFores Algorithm, it is apparent that the deviation of ages converges to the mean and that the deviation of the estimated age decreases compared to the real age. 

% \textcolor{red}{Change the order of the graphs, structure them better after type. Consider integrating them all in one graph.}
% \begin{figure}[h]
% \label{fig:Missforest_Visual_Evaluation}
%   \centering
%     \includegraphics[width=\linewidth]{figs/MissForest_amputation_visual evaluation.png}
%   \caption{Visualization of KDP, BoxPlot, Violin Plot, QQ Plot, Scatter Plott and ECDF Plot of original and imputed age distributions, to evaluate the MissForest() amputation capabilities}
%   \label{fig:MissForest()VisualEvaluation}
% \end{figure}

% \begin{figure}[h]
% \label{fig:VAE}
%   \centering
%     \includegraphics[width=\linewidth]{figs/VAE_amputation_visual evaluation.png}
%   \caption{Visualization of KDP, BoxPlot, Violin Plot, QQ Plot, Scatter Plott and ECDF Plot of original and imputed age distributions, to evaluate the MissForest() amputation capabilities}
%   \label{fig:CVAE()VisualEvaluation}
% \end{figure}

Even though over 80 features are included in the CVAE training and the MissForest imputation training. It is expected that some are more relevant for the model prediction than others. Fortunately, the amputation process also enables a calculation of the individual feature contribution. All features can be ranked after their contribution through the iterative random permutation of all features and recalculation of performance scores, such as R2 or mean squared error. 

Figure XX highlights the 20 most important features relevant to age imputation for both VAE and MissForest. Differentiation between different component types, as well as some categories in the failure reason and type, are most important for age imputation. This is reasonable and motivates the integration of further features, such as more detailed information about the component types in the Analysis. Future work should consider integrating more features to improve age estimation. 

Interestingly, this might also contribute to the 

\subsection{Amputation of Missing Installation Age}

Missing cable age information in the failure report is not the only information that contains data scarcity issues. 

Another piece of information that is hard to obtain is the installation date of the underground cables. If not tracked properly after installation, it is often impossible or not economically feasible to obtain the information. 

However, it can be expected that some other available asset information, such as cable type, diameter, etc., can provide an indication of the installation date of the cable. 


\subsection{Amputation of Missing Loading information}
\textcolor{red}{Present here the amputation of other missing information, such as loading information}

The Loading condintion of the medium voltage cables are relevant for the reliability assessment of the cables, as they represent one potential ageing driver. 

However, regarding the collection of loading information several issues emerge. 

Historrically loading information on medium voltage lines was only collected for important parts of the grid. 



\subsection{Imputation of Missing age information}
\textcolor{red}{Apply the process of missing values on unseen data. Show that the process works. Describe required efforts, such as alignment of encodings for training and application data. Compare the imputation results with other missing value imputation techniques such as miss forest and KNNImputation. Showcase benefits for the probability of failure prediction using only "complete" data vs using complete plus "imputed" data. }

Compared to the MissForest Imputation the VAE requires
the assignment of median and mode values before fulfilling the reconstruction. For this the 



\subsection{Discussion: title might be removed later}
\textcolor{red}{List ideas for the discussion part: Further elaboration} 

This study revealed several pathways for further exploration of VAE-based data enrichment of power grid failure data. Primarily, future work could incorporate more sophisticated sampling methods within the process of missing value imputation. Existing techniques such as Advanced Coupled- Metropolis-within-Gibbs (AC-MWG) and XXX (LIAR) represent thereby high elaboration potential.   

This work applied VAE to medium voltage cable failures. However, for such failures the amount and complexity of training data is limited. Future work could, therefore, apply similar techniques to low-voltage cable failure reports or fusion of the medium-voltage failure dataset with other datasets, such as asset registers or GIS-based features. This might be beneficial, as it can be expected that with a more complex dataset the benefits of the representation learning of the VAE will also increase. For instance, asset data of cables that have not failed, or loading information, could provide additional perspectives when required. This would allow us to create a more holistic model that accounts for various operational conditions and failure modes.

One advantage of using VAEs for the imputation of missing values might be the capability of imputing missing categorical and continious features at the same time. Other imputation techniques, such as MissForest, are also capable of doing so but require further data processing steps to hanlde to different data types. 

\textcolor{red}{Discuss challenges in validating the proof of concept model improvements.} 

\textcolor{red}{Add further parameters to the VAE to improve its capabilities of } 

\textcolor{red}{
Another promising direction is to apply Variational Autoencoders (VAEs) on other types of data relevant for the development of reliability models in power grid components. 
Privacy concerns represent a significant barrier in the utilization of sensitive data for such models. Future work could focus on overcoming this obstacle by decoupling the decoder and encoder components of the VAE through relative representations. Alternatively, other privacy-preserving techniques could be employed to protect sensitive information while still benefiting from the model’s capabilities.
Extending the scope of the current work, the same principles and methods could be applied to low voltage cables. Data scarcity might be an even more critical issue in this area, making the role of sophisticated data imputation and augmentation techniques even more crucial.
The implementation of data enrichment processes based on VAEs also requires specialized tools that facilitate user interaction and data assembly visualization. This would make the model more accessible and interpretable for those without a technical background, thereby promoting broader adoption and understanding.
Finally, Explainable Artificial Intelligence (XAI) techniques could be implemented to better understand the behavior of the VAE models. It might be possible to glean more insights into failure data distributions through VAE representation visualization. This could also aid in the interpretability of the model, making it easier to understand the variables and conditions contributing to specific outcomes.
In summary, the areas for future work are manifold and range from methodological enhancements to applied extensions and ethical considerations. The implementation of these ideas could significantly advance the field, offering more reliable and comprehensive models for power grid reliability.
}

High quality data does not serve a purpose by itself. Therefore one future direction might be to integrate ML classification tasks, such as POF prediction through logistic regressions or even other self supervised learning tasks into the VAE model structure. 

The VAE model requires complete data for training and testing. 
The cleaning of the data however comes with the risk that some categorical features are filtered out. This implies that their representation cannot be learned from the VAE. This risk of a lower variance in the representation of the 
Future work should thus ensure that a sufficient amount of high quality training data is available and that. 

